A simple method to measure numax for asteroseismology: application to 16,000 oscillating Kepler red giants

The importance of numax (the frequency of maximum oscillation power) for asteroseismology has been demonstrated widely in the previous decade, especially for red giants. With the large amount of photometric data from CoRoT, Kepler and TESS, several automated algorithms to retrieve numax values have been introduced. Most of these algorithms correct the granulation background in the power spectrum by fitting a model and subtracting it before measuring numax. We have developed a method that does not require fitting to the granulation background. Instead, we simply divide the power spectrum by a function of the form nu^-2, to remove the slope due to granulation background, and then smooth to measure numax. This method is fast, simple and avoids degeneracies associated with fitting. The method is able to measure oscillations in 99.9% of previously-studied Kepler red giants, with a systematic offset of 1.5 % in numax values that that we are able to calibrate. On comparing the seismic radii from this work with Gaia, we see similar trends to those observed in previous studies. Additionally, our values of width of the power envelope can clearly identify the dipole mode suppressed stars as a distinct population, hence as a way to detect them. We also applied our method to stars with low (0.19--18.35 muHz) and found it works well to correctly identify the oscillations.

==> figures/table.tex <==

\begin{tabular}{cccccccccc}
\toprule
KIC & $K_{\rm p}$ &  $\rm \nu_{max, Yu+2018}$ ($\rm\mu$Hz) & $\rm \Delta\nu$ ($\rm\mu$Hz) & $T_{\rm eff}$ (K) & Phase & \newtwo{$\rm \nu_{max}$} ($\rm\mu$Hz) & \newtwo{$\rm \nu_{max, uncorr}$} ($\rm\mu$Hz) & $P_{\rm peak}$ ($\rm ppm^{2}/ \mu$Hz)  & $W$ ($\rm\mu$Hz) \\
\midrule
 757137 &  9.20 &              29.99 $\pm$ 0.60 &  3.40 $\pm$  0.01 &  4751 $\pm$    139 &        1 &  \newtwo{29.27 $\pm$ 0.44 (QtoQ) $\pm$ 0.33 (MC)} &       31.00 $\pm$     0.43 &     13880 $\pm$      410 &  16.65 $\pm$         0.48 \\
 892010 & 11.67 &               17.85 $\pm$    0.89 &  2.43 $\pm$ 0.08 &  4834 $\pm$    151 &        0 &  \newtwo{17.57 $\pm$      0.33 (QtoQ) $\pm$ 0.36 (MC)}   &    18.35 $\pm$      0.13 &     61500 $\pm$      4900 &   9.00$\pm$        0.91 \\
 892738 & 11.73 &              7.48 $\pm$    0.35 &  1.30 $\pm$  0.03 &  4534 $\pm$   135 &        0 &  \newtwo{7.50 $\pm$      0.12 (QtoQ) $\pm$ 0.14 (MC)}    &   7.91 $\pm$      0.12 &    429600 $\pm$    27000 &   4.51 $\pm$        0.15 \\
 892760 & 13.23 &                29.48 $\pm$    0.48 &  3.96$\pm$ 0.12 &  5188 $\pm$    183 &        2 &  \newtwo{29.10 $\pm$      0.49 (QtoQ) $\pm$ 0.44 (MC)}  &    31.12 $\pm$     1.00 &     19100 $\pm$      1800 &  17.95 $\pm$        3.57 \\
 893214 & 12.58 &                41.39 $\pm$    0.54 &  4.31$\pm$ 0.01 &  4728 $\pm$     80 &        1 & \newtwo{39.88 $\pm$      0.39 (QtoQ) $\pm$ 0.45 (MC)}   &    41.85 $\pm$     0.46 &      6670 $\pm$       300 &  20.33 $\pm$         0.81 \\
 893233 & 11.44 &                  6.15 $\pm$    0.12 &  1.18 $\pm$  0.02 &  4207 $\pm$    147 &        0 & \newtwo{6.20 $\pm$      0.14 (QtoQ) $\pm$ 0.13 (MC)}     &   6.51 $\pm$      0.14 &   1000000 $\pm$     75000 &   3.63 $\pm$        0.16 \\
1026084 & 12.14 &              41.17 $\pm$    0.90 &  4.41$\pm$  0.06 &  5072 $\pm$    166 &        2 & \newtwo{45.10 $\pm$      0.89 (QtoQ) $\pm$ 0.54 (MC)}    &   48.33 $\pm$      0.67 &      3100 $\pm$       120 &  27.35 $\pm$         1.19 \\
1026180 & 11.74 &                36.91 $\pm$    0.71 &  3.99 $\pm$  0.06 &  4718 $\pm$    148 &        2 & \newtwo{35.54 $\pm$      0.60 (QtoQ) $\pm$ 0.51 (MC)}   &    36.83 $\pm$      0.55 &     15000 $\pm$     1400 &  15.72 $\pm$         0.99 \\
1026309 & 10.60 &             16.86 $\pm$    0.76 &  1.93 $\pm$  0.03 &  4514 $\pm$     80 &        0 & \newtwo{16.31 $\pm$      0.33 (QtoQ) $\pm$ 0.28 (MC)}   &     17.54 $\pm$      0.32 &     36000 $\pm$      2300 &  10.91 $\pm$         0.50 \\
1026326 & 13.26 &             94.86 $\pm$    0.65 &  8.83 $\pm$  0.02 &  5123 $\pm$    162 &        1 & \newtwo{94.01 $\pm$      0.41 (QtoQ) $\pm$ 0.46 (MC)}   &     96.61 $\pm$      0.41 &      1500 $\pm$        54 &  34.05$\pm$         1.37 \\
1026452 & 12.94 &               34.50 $\pm$    0.52 &  3.97 $\pm$  0.08 &  5089 $\pm$    154 &        2 & \newtwo{33.82 $\pm$      0.38 (QtoQ) $\pm$ 0.34 (MC)}   &    35.67 $\pm$      0.24 &      9500 $\pm$       400 &  18.36 $\pm$         0.82 \\
1027110 & 12.10 &                6.62 $\pm$    0.19 &  1.15 $\pm$ 0.02 &  4190 $\pm$     80 &        0 & \newtwo{6.48 $\pm$      0.11 (QtoQ) $\pm$ 0.12 (MC)}   &     6.78 $\pm$      0.11 &    860000 $\pm$     60000 &   3.72 $\pm$         0.17 \\
1027337 & 12.11 &                74.21 $\pm$    0.68 &  6.94 $\pm$  0.01 &  4671 $\pm$     80 &        1 &  \newtwo{73.24 $\pm$      0.52 (QtoQ) $\pm$ 0.61 (MC)}   &   75.99 $\pm$      0.54 &      2800 $\pm$       100 &  31.28 $\pm$         0.84 \\
1027582 & 13.88 &               157.75 $\pm$    1.06 & 12.63 $\pm$  0.02 &  5039 $\pm$   155 &        1 & \newtwo{157.34 $\pm$      0.57 (QtoQ) $\pm$ 0.65 (MC)}   &   160.22 $\pm$      0.58 &       708 $\pm$        39 &  45.19 $\pm$         1.62 \\
1028267 & 13.28 &              103.13 $\pm$    0.83 &  9.47 $\pm$  0.02 &  5242$\pm$    183 &        1 &  \newtwo{103.06 $\pm$      1.06 (QtoQ) $\pm$ 0.56 (MC)}   &  106.30 $\pm$      0.80 &      1301 $\pm$        48 &  39.43 $\pm$         1.68 \\
1160684 & 14.91 &              26.38 $\pm$    0.97 &  3.36$\pm$  0.22 &  4128 $\pm$    128 &        2 &  \newtwo{26.71 $\pm$      0.34 (QtoQ) $\pm$ 0.31 (MC)}     & 28.29 $\pm$      0.32 &     17700 $\pm$      1100 &  15.29 $\pm$         0.51 \\
1160789 &  9.70 &              24.72 $\pm$    0.62 &  3.51 $\pm$  0.05 &  4724 $\pm$     80 &        2 &  \newtwo{24.47 $\pm$      0.31 (QtoQ) $\pm$ 0.38 (MC)}      &26.23 $\pm$      0.31 &     28700 $\pm$       940 &  15.58 $\pm$         0.45 \\
1161447 & 12.61 &               36.18 $\pm$    1.55 &  4.12$\pm$  0.06 &  4793 $\pm$     80 &        2 & \newtwo{37.01 $\pm$      0.49 (QtoQ) $\pm$ 0.44 (MC)}     &  39.11 $\pm$      0.41 &      9500 $\pm$       700 &  20.34 $\pm$         0.83 \\
1161618 & 10.22 &               34.32 $\pm$   0.50 &  4.11 $\pm$  0.03 &  4747 $\pm$     80 &        2 & \newtwo{33.62 $\pm$      0.81 (QtoQ) $\pm$ 0.26 (MC)}    &   35.44 $\pm$      0.46 &     14900 $\pm$       740 &  18.17 $\pm$         1.12 \\
1162220 & 11.22 &               11.00 $\pm$    0.32 &  1.67 $\pm$ 0.02 &  4218 $\pm$     80 &        1 & \newtwo{10.91 $\pm$      0.16 (QtoQ) $\pm$ 0.17 (MC)}     &  11.50 $\pm$      0.17 &    248000 $\pm$     15000 &   6.42 $\pm$         0.26 \\
\bottomrule
\end{tabular}

